Caracterizaci\'on Formal y An\'alisis Emp\'irico de Mecanismos Incrementales de B\'usqueda basados en Contexto

The Web has become a potentially infinite information resource, turning into an essential tool for many daily activities. This resulted in an increase in the amount of information available in users' contexts that is not taken into account by current information retrieval systems. This thesis proposes a semisupervised information retrieval technique that helps users to recover context relevant information. The objective of the proposed technique is to reduce the vocabulary gap existing between the knowledge a user has about a specific topic and the relevant documents available in the Web. This thesis presents a method for learning novel terms associated with a thematic context. This is achieved by identifying those terms that are good descriptors and good discriminators of the user's current thematic context. In order to evaluate the proposed method, a theoretical framework for the evaluation of search mechanisms was developed. This served as a guide for the implementation of an evaluation framework that allowed to compare the techniques proposed in this thesis with other techniques existing in the literature. The experimental evidence indicates that the methods proposed in this thesis present significant improvements over previously published techniques. In addition, the evaluation framework was equipped with novel evaluation metrics that favor the exploration of novel material and incorporates a semantic relationship metric between documents. The algorithms developed in this thesis evolve high quality queries, which have the capability of retrieving results that are relevant to the user context. These results have a positive impact on the way users interact with available resources.

==> abstract_en.tex <==
% La Web se ha vuelto un recurso potencialmente infinito de información, transformándose además en una herramienta imprescindible para muchas tareas de la vida diaria.
The Web has become a potentially infinite information resource, turning into an essential tool for many daily  activities.
% Esto provocó un aumento en la cantidad de información existente en el contexto de los usuarios, que no es tenida en cuenta por los sistemas de recuperación de información actuales.
This resulted in an increase in the amount of information available in users' contexts that is not taken into account by current information retrieval systems.
% En esta tesis se propone una técnica semisupervisada de recuperación de información que ayuda al usuario a recuperar información relevante para su contexto actual.
This thesis proposes a semisupervised information retrieval technique that helps users to recover context relevant information.
% El objetivo de la misma es contrarrestar la diferencia de vocabulario que pudiera existir entre el conocimiento que tiene el usuario sobre un tema y los documentos relevantes que se encuentran en la Web.
The objective of the proposed technique is to reduce the vocabulary gap existing between the knowledge a user has about a specific topic and the relevant documents available in the Web.
% Esta tesis presenta un método de aprendizaje de nuevos términos asociados a un contexto temático, a través de la identificación de términos que sean buenos descriptores y términos que sean buenos discriminadores del tópico del contexto actual del usuario.
This thesis presents a method for learning novel terms associated with a thematic context. This is achieved by identifying those terms that are good descriptors and good discriminators of the user’s current thematic context.
% Para la evaluación del método propuesto se desarrolló un marco teórico de evaluación de mecanismos de búsqueda.  Esto dio lugar a la implementación de una plataforma de evaluación, que  permitió comparar las técnicas desarrolladas en esta tesis con otras técnicas existentes en la literatura.
In order to evaluate the proposed method, a theoretical framework for the evaluation of search mechanisms was developed. This served as a guide for the implementation of an evaluation framework that allowed to compare the techniques proposed in this thesis with other techniques existing in the literature.
% La evidencia experimental indica que las mejoras alcanzadas por los métodos propuestos en esta tesis son significativas respecto de las técnicas descriptas en otros trabajos publicados.
The experimental evidence indicates that the methods proposed in this thesis present significant improvements over previously published techniques.
% Dentro de este marco se desarrollaron asimismo nuevas métricas de evaluación que favorecen la exploración de material novedoso y que incorporan una medida de relación semántica entre documentos. 
In addition the evaluation framework was equipped with novel evaluation metrics that favor the exploration of novel material and incorporates a semantic relationship metric between documents. 
% Los algoritmos desarrollados a la largo de esta tesis evolucionan consultas de alta calidad, permitiendo recuperar recursos relevantes al contexto del usuario. Estos resultados impactan positivamente en la forma en la que el usuario interactúa con los recursos que tiene disponibles.
The algorithms developed in this thesis evolve high quality queries, which have the capability of retrieving results that are relevant to the user context. These results have a positive impact on the way users interact with available resources. 

==> abstract_es.tex <==
La Web se ha vuelto un recurso potencialmente infinito de información, transformándose además en una herramienta imprescindible para muchas tareas de la vida diaria. Esto provocó un aumento en la cantidad de información existente en el contexto de los usuarios, que no es tenida en cuenta por los sistemas de recuperación de información actuales.
%  contextual que puede disponer un sistema de recuperación de información y que no tiene en cuenta. 
%
En esta tesis se propone una técnica semisupervisada de recuperación de información que ayuda al usuario a recuperar información relevante para su contexto actual. El objetivo de la misma es contrarrestar la diferencia de vocabulario que pudiera existir entre el conocimiento que tiene el usuario sobre un tema y los documentos relevantes que se encuentran en la Web. Esta tesis presenta un método de aprendizaje de nuevos términos asociados a un contexto temático, a través de la identificación de términos que sean buenos descriptores y términos que sean buenos discriminadores del tópico del contexto actual del usuario.
% respondiendo a si este puede explotarse para acceder a material relevante
Para la evaluación del método propuesto se desarrolló un marco teórico de evaluación de mecanismos de búsqueda y se implementó una plataforma de evaluación, que además permitió comparar las técnicas desarrolladas en esta tesis
con otras técnicas existentes en la literatura. La evidencia experimental muestra que las mejoras alcanzadas son significativas respecto de otros trabajos publicados.
% métricas
Dentro de este marco se desarrollaron asimismo nuevas métricas de evaluación que favorecen la exploración de material novedoso y que incorporan una medida de relación semántica entre documentos.
%
Los algoritmos desarrollados a la largo de esta tesis evolucionan consultas de alta calidad, permitiendo recuperar recursos relevantes al contexto del usuario, e impactan positivamente en la forma en la que éste interactúa con los recursos que tiene disponibles.
